Time-Optimal Collision Avoidance Via a Greedy Polynomial Backward Sweep

Spacecraft collision avoidance for low-thrust satellites often requires determining not only how to maneuver, but also how late a maneuver can begin while still ensuring safety. This paper presents a greedy time-optimal (GTO) backward-sweep method to find the latest maneuver initiation time. The method starts from the nominal time of closest approach and iteratively propagates the maneuver backward in time, selecting at each step the thrust direction that locally minimizes the chosen danger metric. Differential algebra is used to efficiently propagate state sensitivities and update the time of closest approach online. The method is tested on a large dataset of conjunctions, using both miss distance and probability of collision as safety metrics. The approach achieves accurate results and only a small loss of optimality relative to an optimal-control benchmark, while retaining runtimes suitable for on-board implementation.

==> Figures/b-plane.tex <==






\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,465); %set diagram left start at 0, and has height of 465

%Straight Lines [id:da1719990401256153] 
\draw [line width=1.5]  [dash pattern={on 5.63pt off 4.5pt}]  (370,238) -- (371,121.67) ;
%Straight Lines [id:da6056213587618334] 
\draw [line width=1.5]  [dash pattern={on 5.63pt off 4.5pt}]  (371,121.67) -- (282.75,87.5) ;
%Straight Lines [id:da21160951945207707] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.75]    (283,203) -- (236.77,29.9) ;
\draw [shift={(236,27)}, rotate = 75.05] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da7666646074688507] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=1.5]    (283,203) -- (368.06,124.38) ;
\draw [shift={(371,121.67)}, rotate = 137.25] [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (11.61,-5.58) -- (0,0) -- (11.61,5.58) -- cycle    ;
%Straight Lines [id:da47921981090746657] 
\draw [line width=1.5]    (283,203) -- (408.29,253.5) ;
\draw [shift={(412,255)}, rotate = 201.95] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (11.61,-5.58) -- (0,0) -- (11.61,5.58) -- cycle    ;
%Shape: Circle [id:dp7100792087747478] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (367.67,121.67) .. controls (367.67,119.83) and (369.16,118.33) .. (371,118.33) .. controls (372.84,118.33) and (374.33,119.83) .. (374.33,121.67) .. controls (374.33,123.51) and (372.84,125) .. (371,125) .. controls (369.16,125) and (367.67,123.51) .. (367.67,121.67) -- cycle ;
%Straight Lines [id:da2872937414839446] 
\draw [line width=1.5]    (283,203) -- (139.87,240) ;
\draw [shift={(136,241)}, rotate = 345.51] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (11.61,-5.58) -- (0,0) -- (11.61,5.58) -- cycle    ;
%Straight Lines [id:da7614184023654675] 
\draw [line width=1.5]    (283,203) -- (283,33) ;
\draw [shift={(283,29)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (11.61,-5.58) -- (0,0) -- (11.61,5.58) -- cycle    ;
%Straight Lines [id:da5741149422048625] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.75]    (283,203) -- (149.98,52.25) ;
\draw [shift={(148,50)}, rotate = 48.58] [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da6917854388377487] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=1.5]    (283,203) -- (198.87,224.99) ;
\draw [shift={(195,226)}, rotate = 345.35] [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (11.61,-5.58) -- (0,0) -- (11.61,5.58) -- cycle    ;
%Shape: Circle [id:dp8022912382599631] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (279.67,203) .. controls (279.67,201.16) and (281.16,199.67) .. (283,199.67) .. controls (284.84,199.67) and (286.33,201.16) .. (286.33,203) .. controls (286.33,204.84) and (284.84,206.33) .. (283,206.33) .. controls (281.16,206.33) and (279.67,204.84) .. (279.67,203) -- cycle ;
%Straight Lines [id:da21867553564150388] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=1.5]    (236,27) -- (151.87,48.99) ;
\draw [shift={(148,50)}, rotate = 345.35] [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (11.61,-5.58) -- (0,0) -- (11.61,5.58) -- cycle    ;

% Text Node
\draw (262.33,26) node [anchor=north west][inner sep=0.75pt]    {$\xi $};
% Text Node
\draw (383.33,250) node [anchor=north west][inner sep=0.75pt]    {$\zeta $};
% Text Node
\draw (151,240) node [anchor=north west][inner sep=0.75pt]    {$\eta $};
% Text Node
\draw (192.33,57) node [anchor=north west][inner sep=0.75pt]    {$\textcolor[rgb]{0.82,0.01,0.11}{v}\textcolor[rgb]{0.82,0.01,0.11}{_{s}}\textcolor[rgb]{0.82,0.01,0.11}{(}\textcolor[rgb]{0.82,0.01,0.11}{t}\textcolor[rgb]{0.82,0.01,0.11}{_{CA}}\textcolor[rgb]{0.82,0.01,0.11}{)}$};
% Text Node
\draw (126.33,80) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$\textcolor[rgb]{0.29,0.56,0.89}{v}\textcolor[rgb]{0.29,0.56,0.89}{_{p}(}\textcolor[rgb]{0.29,0.56,0.89}{t}\textcolor[rgb]{0.29,0.56,0.89}{_{CA}}\textcolor[rgb]{0.29,0.56,0.89}{)}$};
% Text Node
\draw (296.33,129) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$\textcolor[rgb]{0.29,0.56,0.89}{r( t_{CA})}$};
% Text Node
\draw (167.33,10) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$\textcolor[rgb]{0.25,0.46,0.02}{v( t_{CA})}$};
% Text Node
\draw (249,213) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textcolor[rgb]{0.82,0.01,0.11}{Secondary}};
% Text Node
\draw (361,92) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textcolor[rgb]{0.29,0.56,0.89}{Primary}};
% Text Node
\draw (204,229) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$\textcolor[rgb]{0.25,0.46,0.02}{v}\textcolor[rgb]{0.25,0.46,0.02}{(}\textcolor[rgb]{0.25,0.46,0.02}{t}\textcolor[rgb]{0.25,0.46,0.02}{_{CA}}\textcolor[rgb]{0.25,0.46,0.02}{)}$};


\end{tikzpicture}


==> algorithm.tex <==
\begin{algorithm}
\footnotesize
\caption{Backward sweep for warning-time optimization of low-thrust \gls{cam}.}
\label{alg:backwardSweep}
\begin{algorithmic}[1]
    \State {Define scenario parameters: $u_{max}$, $\gamma$, $t_{\mathrm{alert}}$, $N$.}
    \State {Get input from conjunction assessment: $\vec{x}$, $\vec{x}_s$, $\vec{P}_p$, $\vec{P}_s$,  $R$.}
    \State {Define the discrete grid $\vec{t}=\{t_{\mathrm{alert}},\ldots,t_{N}=t_{\mathrm{CA}}\}$ with $N+1$ nodes.}
    \State {$i \gets N$.}
    \While{$\bar{d}_{(\cdot)^{(i)}} < \gamma$  \&  $i > 0$}
        \State {$\bar{\vec{x}}_{i-1} \gets$ \cref{eq:backPropi}: propagate backwards}
        \State {$\vec{x}_{i-1} \gets$ \cref{eq:exp_state}: expand the state around the nominal value.}
        \If{$i = N$}
            % \State {$\vec{x}_{s,N} \gets \mathcal{T}_{\vec{x}_{s,N}}(\delta t)$: Perturb the dynamics of the secondary around \gls{tca}.}
            \State {$\vec{x}_{N} \gets$: \cref{eq:StateTaylorsp} propagate forwards using \gls{da} perturbations in state, control, and \gls{tca}.}
            \State {$\vec{x}_{s,N} \gets$: \cref{eq:StateTaylorss} propagate forwards secondary using \gls{da} perturbations in state, control, and \gls{tca}.}
            \State {$\delta t \gets $ \cref{eq:deltaT}: Invert the polynomial for \gls{tca} condition.}
            \State {$\vec{r}_{\mathcal{B}}\gets$ \cref{eq:expBplane}.}
            \State {$d_{(\cdot)}\gets$\cref{eq:DMTaylor}.}
        \Else
            \State {$\delta\vec{x}_{i} \gets$: \cref{eq:TaylorsBack_i} propagate \gls{da} perturbations.}
            \State {$\delta t^{(i)} \gets \mathcal{T}_{\delta t}(\delta\vec{x}_{i-1},\delta\vec{u}_{i-1})$ .}
            % \State {$\vec{r}_{\mathcal{B}}\gets \mathcal{T}_{\vec{r}_{\mathcal{B}}}(\delta\vec{x}_{i-1},\delta\vec{u}_{i-1})$.}
            % \State {$\vec{\Sigma}_{\mathcal{B}}\gets \mathcal{T}_{\vec{\Sigma}_{\mathcal{B}}}(\delta\vec{x}_{i-1},\delta\vec{u}_{i-1})$.}
            \State {$d_{(\cdot)}^{(i)}\gets \mathcal{T}_{d_{(\cdot)}}(\delta\vec{x}_{i-1},\delta\vec{u}_{i-1})$.}
        \EndIf
        \If{$\bar{d}_{(\cdot)}^{(i)} > \gamma$}
            \State{$\vec{x}_{N-i}\gets$ \cref{eq:backProp_j}.}
            \State{$\vec{x}_{N-i+1}\gets$ \cref{eq:T_j}.}
            \State{$\tau\gets$ \cref{eq:tau}.}
            \State{$\bar{t}_{N-j}\gets\bar{t}_{N-j}-\tau$.}
            \State{$\bar{d}_{(\cdot)}^{(i)}\gets$.}
            \State{$\bar{t}_{CA}^{(i)}\gets$.}
            
        \EndIf
        \State{$\vec{u}_{i-1} \gets$ \cref{eq:Control_i}: greedy control.} %should include update of the maps with control but don't know how to write it
        \State{$i \gets i-1$.}
    \EndWhile
\end{algorithmic}
\end{algorithm}

==> glossary.tex <==
\newacronym{leo}{LEO}{low Earth orbit}
\newacronym{geo}{GEO}{geostationary Earth orbit}
\newacronym{smd}{SMD}{squared Mahalanobis distance}
\newacronym{md}{MD}{miss distance}
\newacronym{ssa}{SSA}{Space Situational Awareness}
\newacronym{adr}{ADR}{Active Debris Removal}
\newacronym{sk}{SK}{station keeping}
\newacronym{ca}{CA}{collision avoidance}
\newacronym{ipc}{IPoC}{instantaneous probability of collision}
\newacronym{tipc}{TIPoC}{total instantaneous probability of collision}
\newacronym{cpc}{CPoC}{cumulative probability of collision}
\newacronym{poc}{PoC}{probability of collision}
\newacronym{tpoc}{TPoC}{total probability of collision}
\newacronym{cam}{CAM}{collision avoidance maneuver}
\newacronym{scvx}{SCvx}{successive convexification}
\newacronym{erf}{erf}{error function}
\newacronym{da}{DA}{differential algebra}
\newacronym{eci}{ECI}{Earth Centered Inertial}
\newacronym{ecef}{ECEF}{Earth Centered Earth Fixed}
\newacronym{lvlh}{LVLH}{Local Vertical Local Horizon}
\newacronym{hbr}{HBR}{hard body radius}
\newacronym{pdf}{PDF}{Probability Density Function}
\newacronym{nlp}{NLP}{nonlinear program}
\newacronym{srp}{SRP}{solar radiation pressure}
\newacronym{mpbvp}{MPBVP}{multi-point boundary value problem}
\newacronym{cw}{CW}{Clohessy-Wiltshire}
\newacronym{ns}{N-S}{North-South}
\newacronym{sdp}{SDP}{Semidefinite program}
\newacronym{qcqp}{QCQP}{Quadratically constrained quadratic program}
\newacronym{qp}{QP}{quadratic program}
\newacronym{zoh}{ZOH}{zeroth-order hold}
\newacronym{oc}{OC}{optimal control}
\newacronym{to}{TO}{time-optimal}
\newacronym{gto}{GTO}{greedy TO}
\newacronym{ocp}{OCP}{optimal control problem}
\newacronym{ew}{E-W}{East-West}
\newacronym{stm}{STM}{state transition matrix}
\newacronym{rtn}{RTN}{radial, along-track, cross-track}
\newacronym{iss}{ISS}{International Space Station}
\newacronym{lp}{LP}{linear program}
\newacronym{gnc}{GNC}{guidance, navigation, and control}
\newacronym{koz}{KOZ}{keep-out-zone}
\newacronym{socp}{SOCP}{second-order cone program}
\newacronym{cp}{CP}{convex program}
\newacronym{mrv}{MRV}{multivariate random variable}
\newacronym{gmm}{GMM}{Gaussian mixture model}
\newacronym{rv}{RV}{random variable}
\newacronym{scp}{SCP}{sequential convex program}
\newacronym{rso}{RSO}{resident space object}
\newacronym{mc}{MC}{Monte Carlo}
\newacronym{mss}{MSS}{Mahalanobis Shell Sampling}
\newacronym{nli}{NLI}{nonlinearity index}
\newacronym{rk}{RK}{Runge-Kutta}
\newacronym{trr}{TRR}{trust region radius}
\newacronym{tca}{TCA}{time of closest approach}
\newacronym{aida}{AIDA}{Accurate Integrator for Debris Analysis}
\newacronym{fo}{FO}{fuel-optimal}
\newacronym{ava}{AvA}{active vs active}
\newacronym{cdm}{CDM}{Conjunction Data Message}
\newacronym{cr3bp}{CR3BP}{circular restricted three-body problem}
\newacronym{pp}{PP}{polynomial program}
\newacronym{stt}{STT}{state transition tensor}
\newacronym{rsw}{RSW}{radial, cross-track, along-track}

